BDDs Strike Back: Efficient Analysis of Static and Dynamic Fault Trees

Fault trees are a key model in reliability analysis. Classical static fault trees (SFT) can best be analysed using binary decision diagrams (BDD). State-based techniques are favorable for the more expressive dynamic fault trees (DFT). This paper combines the best of both worlds by following Dugan's approach: dynamic sub-trees are analysed via model checking Markov models and replaced by basic events capturing the obtained failure probabilities. The resulting SFT is then analysed via BDDs. We implemented this approach in the Storm model checker. Extensive experiments (a) compare our pure BDD-based analysis of SFTs to various existing SFT analysis tools, (b) indicate the benefits of our efficient calculations for multiple time points and the assessment of the mean-time-to-failure, and (c) show that our implementation of Dugan's approach significantly outperforms pure Markovian analysis of DFTs. Our implementation Storm-dft is currently the only tool supporting efficient analysis for both SFTs and DFTs.

==> dft-tikz.tex <==

\makeatletter

\pgfdeclareshape{spare}{
  % The 'minimum width' and 'minimum height' keys, not the content, determine
  % the size
  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  % This is redundant, but makes some things easier:
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  % Inherit from rectangle
  \inheritanchorborder[from=rectangle]

  % Define same anchor a normal rectangle has
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{\northeast}
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  % Define anchors for signal ports
  \anchor{O}{ % output anchor
    \pgf@process{\northeast}%
    \pgf@x=0pt%
  }
  \anchor{P}{ % primary anchor
    \pgf@process{\northeast}%
    \pgf@x=-.5\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SA}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.1\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SB}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.3\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SC}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.5\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SD}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.7\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SE}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.9\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{BOX}{ % spare box anchor
    \pgf@process{\northeast}%
    \pgf@x=\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{LINE}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.\pgf@y%
  }
  % Draw the rectangle box and the port labels
  \backgroundpath{
    % Rectangle box
    \pgfpathrectanglecorners{\southwest}{\northeast}
    % Line in the middle
    \pgf@anchor@spare@LINE
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \advance\pgf@xb by -2\pgf@x
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    % Box for spare parts
    \pgf@anchor@spare@BOX
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@xc=\pgf@x \pgf@yc=\pgf@y
    \advance\pgf@ya by -.\pgf@y
    \advance\pgf@yb by -.8\pgf@y
    \advance\pgf@xb by -1\pgf@x
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    \pgfclosepath

    % Draw port labels
    \begingroup
    \tikzset{spare/port labels} % Use font from this style
    \tikz@textfont

    \pgf@anchor@spare@O
    \pgftext[top,at={\pgfpoint{\pgf@x}{\pgf@y}},y=-\pgfshapeinnerysep]{}

    \pgf@anchor@spare@P 
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SA
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SB
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SC
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SD
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SE
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    \endgroup
  }
}

\tikzset{add font/.code={\expandafter\def\expandafter\tikz@textfont\expandafter{\tikz@textfont#1}}} 

\tikzset{spare/port labels/.style={font=\sffamily\scriptsize}}
\tikzset{every spare node/.style={draw,minimum height=1cm,minimum 
width=1.5cm,fill=white!100!black,inner sep=1mm,outer sep=0pt,cap=round,add 
font=\sffamily}}

\pgfdeclareshape{spareM}{
  % The 'minimum width' and 'minimum height' keys, not the content, determine
  % the size
  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  % This is redundant, but makes some things easier:
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  % Inherit from rectangle
  \inheritanchorborder[from=rectangle]

  % Define same anchor a normal rectangle has
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{\northeast}
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  % Define anchors for signal ports
  \anchor{O}{ % output anchor
    \pgf@process{\northeast}%
    \pgf@x=0pt%
  }
  \anchor{P}{ % primary anchor
    \pgf@process{\northeast}%
    \pgf@x=.5\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SA}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=-.1\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SB}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=-.3\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SC}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=-.5\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SD}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=-.7\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SE}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.9\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{BOX}{ % spare box anchor
    \pgf@process{\northwest}%
    \pgf@x=\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{LINE}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.\pgf@y%
  }
  % Draw the rectangle box and the port labels
  \backgroundpath{
    % Rectangle box
    \pgfpathrectanglecorners{\southwest}{\northeast}
    % Line in the middle
    \pgf@anchor@spare@LINE
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \advance\pgf@xb by -2\pgf@x
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    % Box for spare parts
    \pgf@anchor@spare@BOX
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@xc=\pgf@x \pgf@yc=\pgf@y
    \advance\pgf@ya by -.\pgf@y
    \advance\pgf@xa by -1\pgf@x
    \advance\pgf@yb by -.8\pgf@y
    \advance\pgf@xb by -2\pgf@x
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    \pgfclosepath

    % Draw port labels
    \begingroup
    \tikzset{spareM/port labels} % Use font from this style
    \tikz@textfont

    \pgf@anchor@spare@O
    \pgftext[top,at={\pgfpoint{\pgf@x}{\pgf@y}},y=-\pgfshapeinnerysep]{}

    \pgf@anchor@spare@P 
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SA
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SB
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SC
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SD
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SE
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    \endgroup
  }
}

\tikzset{add font/.code={\expandafter\def\expandafter\tikz@textfont\expandafter{\tikz@textfont#1}}} 

\tikzset{spareM/port labels/.style={font=\sffamily\scriptsize}}
\tikzset{every spareM node/.style={draw,minimum height=1cm,minimum 
width=1.5cm,inner sep=1mm,outer sep=0pt,cap=round,add 
font=\sffamily}}

\pgfdeclareshape{fdep}{
  % The 'minimum width' and 'minimum height' keys, not the content, determine
  % the size
  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  % This is redundant, but makes some things easier:
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  % Inherit from rectangle
  \inheritanchorborder[from=rectangle]

  % Define same anchor a normal rectangle has
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{\northeast}
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  % Define anchors for signal ports
  \anchor{O}{ % output anchor
    \pgf@process{\northeast}%
    \pgf@x=0pt%
  }
  \anchor{EA}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.1\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{EB}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.3\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{EC}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.5\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{ED}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.7\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{EE}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.9\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{T}{ % trigger anchor
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.5\pgf@y%
  }
  \anchor{LINE}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.\pgf@y%
  }
  % Draw the rectangle box and the port labels
  \backgroundpath{
    % Rectangle box
    \pgfpathrectanglecorners{\southwest}{\northeast}
    % Line in the middle
    \pgf@anchor@fdep@LINE
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \advance\pgf@xb by -2\pgf@x
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    % trinagle input
    \pgf@anchor@fdep@T
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@xc=\pgf@x \pgf@yc=\pgf@y
    \advance\pgf@ya by -.3333\pgf@x
    \advance\pgf@xb by -.5\pgf@x
    \advance\pgf@yb by .\pgf@x
    \advance\pgf@yc by .3333\pgf@x
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
    \pgfclosepath

    % Draw port labels
    \begingroup
    \tikzset{fdep/port labels} % Use font from this style
    \tikz@textfont

    \pgf@anchor@fdep@O
    \pgftext[top,at={\pgfpoint{\pgf@x}{\pgf@y}},y=-\pgfshapeinnerysep]{}
    
    \pgf@anchor@fdep@EA
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@fdep@EB
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@fdep@EC
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@fdep@ED
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@fdep@EE
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    \endgroup
  }
}

\tikzset{add font/.code={\expandafter\def\expandafter\tikz@textfont\expandafter{\tikz@textfont#1}}} 

\tikzset{fdep/port labels/.style={font=\sffamily\scriptsize}}
\tikzset{every fdep node/.style={draw,minimum height=1cm,minimum 
width=1.5cm,inner sep=1mm,outer sep=0pt,cap=round,add 
font=\sffamily}}

\newif\ifpgfshapebaselesstrianglehasinline
\newif\ifpgfshapebaselesstriangleclose
\pgfkeys{/pgf/.cd,
  baseless triangle apex angle/.style={/pgf/isosceles triangle apex angle=#1},
  baseless triangle inline/.is if=pgfshapebaselesstrianglehasinline,
  baseless triangle has base/.is if=pgfshapebaselesstriangleclose
}

\pgfdeclareshape{baseless triangle}{
  % Copy some stuff from the isosecles triangle
  \inheritsavedanchors[from={isosceles triangle}]
  \inheritanchor[from={isosceles triangle}]{center}
  \inheritanchor[from={isosceles triangle}]{north}
  \inheritanchor[from={isosceles triangle}]{south}
  \inheritanchor[from={isosceles triangle}]{east}
  \inheritanchor[from={isosceles triangle}]{west}
  \inheritanchorborder[from={isosceles triangle}]
  \backgroundpath{%
    % The isoceles triangle defines lots of parameters
    % in the \trianglepoints macro.
        \trianglepoints%
        {%
            \pgftransformshift{\centerpoint}%
            \pgftransformrotate{\rotate}%
            % This bit is a bit of a kludge to ensure the inline
            % is at the top of the figure.
            \pgftransformyscale{cos(\rotate)}%
            \pgfpathmoveto{\lowerleft}%
            \pgfpathlineto{\apex}%
            \pgfpathlineto{\lowerleft\pgf@y=-\pgf@y}%
            % Close the base?
            \ifpgfshapebaselesstriangleclose%
              \pgfpathclose%
            \fi%
            % Draw the inline?
            \ifpgfshapebaselesstrianglehasinline
              \pgfpointdiff{\lowerleft}%
                 {\pgfpointlineattime{0.125}{\lowerleft}{\lowerleft\pgf@y=-\pgf@y}}%
                \pgfgetlastxy{\x}{\y}%
                \pgfmathveclen{\x}{\y}%
                \let\inlineshift=\pgfmathresult%
            % Calculate where the inline hits the sloped line of the triangle.
            \pgfmathparse{\inlineshift/2/sin(\pgfkeysvalueof{/pgf/isosceles triangle apex angle}/2)}%
            \let\inlineendshift=\pgfmathresult
            \pgfpathmoveto{\pgfpointadd{\pgfpoint{0pt}{-\inlineshift}}{\lowerleft}}%
            \pgfpathlineto{\pgfpointlineatdistance{\inlineendshift}{\apex}{\lowerleft}\pgf@y=-\pgf@y}%
        \fi%
    }
    }
}





\makeatother

\tikzstyle{every picture}=[>=stealth]
\tikzstyle{fdarrow}=[>=triangle 60,double,double equal sign distance,-implies,dashed]
\tikzstyle{and1}=[and gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=n,minimum width=1cm]
\tikzstyle{and2}=[and gate US,draw,  shape border rotate=90, rotate=90,logic gate inputs=nn,minimum width=1cm]
\tikzstyle{and3}=[and gate US,draw, shape border rotate=90, rotate=90,logic gate inputs=nnn,minimum width=1cm]
\tikzstyle{and}=[and gate US,draw, shape border rotate=90, rotate=90,logic gate inputs=nnn,minimum width=1cm]
\tikzstyle{and4}=[and gate US,draw, shape border rotate=90, rotate=90,logic gate inputs=nnnn,minimum width=1cm, scale=0.9]
\tikzstyle{and5}=[and gate US,draw, shape border rotate=90, rotate=90,logic gate inputs=nnnnn,minimum width=1cm, scale=0.8]
\tikzstyle{and6}=[and gate US,draw, shape border rotate=90, rotate=90,logic gate inputs=nnnnnn,minimum width=1cm, scale=0.7]
\tikzstyle{or1}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=n,minimum width=1cm]
\tikzstyle{or2}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=nn,minimum width=1cm]
\tikzstyle{or3}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=nnn,minimum width=1cm]
\tikzstyle{or}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=nnn,minimum width=1cm]
\tikzstyle{or4}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=nnnn,minimum width=1cm, scale=0.9]
\tikzstyle{or5}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=nnnnn,minimum width=1cm, scale=0.8]
\tikzstyle{or6}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=nnnnnn,minimum width=1cm, scale=0.8]
\tikzstyle{be}=[circle,draw,fill=white!100,anchor=north, inner sep=5pt, minimum width=0.7cm]
\tikzstyle{cnst}=[diamond,draw,fill=white!100,anchor=north, minimum width=0.5cm,font=\scriptsize, scale=0.8]
\tikzstyle{seq}=[rectangle, draw, fill=white!100, minimum width=1.0cm, minimum height=0.6cm, inner sep=3pt, label=center:{\LARGE$\rightarrow$}]
\tikzstyle{seqincl}=[seq, label={[shift={(0.35,-0.65)}]\small{$\leq$}}]
\tikzstyle{seqexcl}=[seq, label={[shift={(0.35,-0.65)}]\small{$<$}}]
\tikzstyle{mutex}=[rectangle, draw, fill=white!100, minimum width=1.0cm, minimum height=0.6cm, inner sep=3pt, label=center:{\LARGE$\leftrightarrow$}]
\tikzstyle{labelbox} = [rectangle, draw, inner sep=2pt, anchor=south, minimum width=0.6cm, minimum height=0.48cm, scale=0.8]
\tikzstyle{ratebox} = [rectangle, draw=none, inner sep=2pt, anchor=north, minimum width=0.6cm, minimum height=0.48cm, scale=0.8, align=center]
\tikzstyle{transfer} = [isosceles triangle, draw, shape border rotate=90, inner sep=2pt, minimum width=0.9cm, minimum height=0.7cm, isosceles triangle stretches=true]

\tikzstyle{triangle}=[isosceles triangle,draw,shape border rotate=90,isosceles triangle stretches=true, minimum height=0.6cm,minimum width=0.6cm]
\tikzstyle{triangle_pand}=[triangle, scale=1.62, yshift=-3.5, xscale=0.80]
\tikzstyle{btriangle}=[baseless triangle,draw,rotate=90, minimum height=0.6cm]
\tikzstyle{triangle_por}=[btriangle, scale=1.62, yscale=0.915, xshift=-0.113cm]

\tikzstyle{subtree}=[triangle]
\tikzstyle{failed}=[draw=red!60!black!100, fill=red!05]

\tikzstyle{repr}=[fill=black!30!white]
% Need to copy style from spare and explicitly set background colour
\tikzstyle{spare_repr}=[spare, every spare node/.style={draw,minimum height=1cm,minimum width=1.5cm,fill=black!30!white,inner sep=1mm,outer sep=0pt,cap=round,add font=\sffamily}]


==> packages.tex <==
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage[english]{babel}
\usepackage{graphicx}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{xspace}
\usepackage{subfigure}
\usepackage{paralist}
\usepackage{booktabs}
\usepackage{csvsimple}
\usepackage{longtable}
\usepackage[binary-units]{siunitx}


% ORCID Symbol
\makeatletter
\RequirePackage[bookmarks,unicode,colorlinks=true]{hyperref}%
\def\@citecolor{blue}%
\def\@urlcolor{blue}%
\def\@linkcolor{blue}%
\def\UrlFont{\rmfamily}
\def\orcidID#1{\smash{\href{https://orcid.org/#1}{\protect\raisebox{-1.25pt}{\protect\includegraphics{orcid_color.pdf}}}}}
\makeatother


%\usepackage{hyperref}
% If you use the hyperref package, please uncomment the following line
% to display URLs in blue roman font according to Springer's eBook style:
\renewcommand\UrlFont{\color{blue}\rmfamily}


\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=1.17}
\usetikzlibrary{shapes.gates.logic.US,shapes.geometric,positioning,fit,calc}
\usepgfplotslibrary{colorbrewer} % Colorbrewer color schemes

\input{dft-tikz}
\input{pgfplots}

\tikzstyle{bdd}=[innernode/.style={draw, circle}, leaf/.style={draw, rectangle}, succzero/.style={draw,dashed}, succone/.style={draw}]


\usepackage{algorithm}
\usepackage[noend]{algpseudocode}

% Input/Output for algorithms
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}


\newcommand\bfpar[1]{%
\medskip\noindent\textbf{#1}}


==> pgfplots.tex <==
\pgfplotsset{
    scatterplot/.style={
        width=5.05cm, height=5.05cm,
        axis x line=bottom, axis y line=left,
        x label style={at={(axis description cs:0.5,-0.14)},anchor=north},
        y label style={at={(axis description cs:-0.18,0.5)},anchor=south},
        yticklabel style={font=\tiny}, xticklabel style={rotate=290, anchor=west, font=\tiny},
        legend pos=north west, legend style={font=\tiny, row sep=-2pt}, legend cell align={left}
    },
    scatterruntime/.style={
        scatterplot,
        xmin=0.001, ymin=0.001, ymax=600, xmax=600,
        log ticks with fixed point,
        %xtick={0.1, 1, 10, 60, 300}, xticklabels={0.1, 1, 10, 60, 300},
        %ytick={0.1, 1, 10, 60, 300}, yticklabels={0.1, 1, 10, 60, 300},
        extra x ticks = {600}, extra x tick labels = {OoR}, extra x tick style = {grid = major},
        extra y ticks = {600}, extra y tick labels = {OoR}, extra y tick style = {grid = major}
    },
}


% Markers for plots
\tikzset{%
    aralia/.style={     Dark2-A,mark=*,mark size=1.30},
    sprinkler/.style={  Dark2-H,mark=pentagon*,  mark size=1.30},
    railway/.style={    Dark2-C,mark=square*,        mark size=1.30},
    industry/.style={   Dark2-D,mark=diamond*, mark size=1.30},
    randomScram/.style={Dark2-F,mark=triangle*,mark size=1.30},
    randomScramProb/.style={Dark2-F,mark=triangle,mark size=1.30},
    %other/.style={      Dark2-B,mark=oplus*,   mark size=1.30},
    %other/.style={      Dark2-H,mark=otimes*,  mark size=1.30},
    modsft/.style={     Dark2-A,mark=triangle*, mark size=1.30},
    modrailway/.style={ Dark2-F,mark=square*, mark size=1.30},
    modvgs/.style={     Dark2-C,mark=*, mark size=1.30},
    ffort/.style={      Dark2-D,mark=diamond*, mark size=1.30},
}


% Diagonal lines
\newcommand*{\diagonalsTimes}{
  \addplot[no marks] coordinates
    {(0.001,0.001) (300,300) };
  \addplot[no marks, dashed] coordinates
    {(0.01,0.001) (300,30) };
  \addplot[no marks, dashed] coordinates
    {(0.1,0.001) (300,3) };
  \addplot[no marks, dashed] coordinates
    {(0.001,0.01) (30,300) };
  \addplot[no marks, dashed] coordinates
    {(0.001,0.1) (3,300) };
}

